Enhancements to ACL2 in Versions 5.0, 6.0, and 6.1

We report on highlights of the ACL2 enhancements introduced in ACL2 releases since the 2011 ACL2 Workshop. Although many enhancements are critical for soundness or robustness, we focus in this paper on those improvements that could benefit users who are aware of them, but that might not be discovered in everyday practice.

==> eptcsdata.tex <==
\providecommand{\firstpage}{5}
\providecommand{\publicationstatus}{R. Gamboa and J. Davis (Eds.): ACL2 Workshop 2013 (ACL2 '13).\\
EPTCS 114, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.114.1}{10.4204/EPTCS.114.1}}
\pdfoutput=1

